A Particle-in-cell Method for Plasmas with a Generalized Momentum Formulation, Part II: Enforcing the Lorenz Gauge Condition

In a previous paper, we developed a new particle-in-cell method for the Vlasov-Maxwell system in which the electromagnetic fields and the equations of motion for the particles were cast in terms of scalar and vector potentials through a Hamiltonian formulation. This paper extends this new class of methods by focusing on the enforcement the Lorenz gauge condition in both exact and approximate forms using co-located meshes. A time-consistency property of the proposed field solver for the vector potential form of Maxwell's equations is established, which is shown to preserve the equivalence between the semi-discrete Lorenz gauge condition and the analogous semi-discrete continuity equation. Using this property, we present three methods to enforce a semi-discrete gauge condition. The first method introduces an update for the continuity equation that is consistent with the discretization of the Lorenz gauge condition. The second approach we propose enforces a semi-discrete continuity equation using the boundary integral solution to the field equations. The third approach introduces a gauge correcting method that makes direct use of the gauge condition to modify the scalar potential and uses local maps for both the charge and current densities. The vector potential coming from the current density is taken to be exact, and using the Lorenz gauge, we compute a correction to the scalar potential that makes the two potentials satisfy the gauge condition. We demonstrate two of the proposed methods in the context of periodic domains. Problems defined on bounded domains, including those with complex geometric features remain an ongoing effort. However, this work shows that it is possible to design computationally efficient methods that can effectively enforce the Lorenz gauge condition in an non-staggered PIC formulation.

==> 2-Formulation/BDF-diffusion-solver.tex <==
%
% Brief intro on the BDF solver for the diffusion equation
%
\subsection{A Semi-discrete BDF Method for Linear Diffusion Equations}

The fourth method we present is a parabolic cleaning method. We use the  parabolic cleaning method to enforce the gauge condition, which is described in section \ref{sec:4 gauge correcting}.  This method requires the solution of a diffusion equation. In previous work on phase-field models, the method-of-lines-transpose was used to develop algorithms with high-order temporal and spatial accuracy for linear and non-linear parabolic equations \cite{causley2016phase-field,causley2017phase-field}. In this work, we shall consider the first-order BDF method introduced in \cite{causley2017phase-field}, which is consistent with the temporal accuracy of the BDF wave solver. Details concerning the accuracy and unconditional stability of these methods can be found in the aforementioned articles. As we shall soon see, the operators that need to be inverted in the diffusion equation are identical in structure to those used in the wave solver. This provides an opportunity to reuse algorithms across applications, a feature that was discussed in our recent work on parallel algorithms \cite{christlieb2020parallel}.

Consider now the linear diffusion equation
\begin{equation}
    \label{eq:diffusion equation}
    \partial_{t} \psi - D \Delta \psi = S.
\end{equation}
The coefficient $D > 0$ represents the scalar diffusivity, which, for our purposes, is assumed to be a constant. Additionally, we use $\Delta$ to denote the Laplacian operator and $S(\mathbf{x},t)$ is the source function. To obtain the first-order semi-discrete scheme for the diffusion equation, we apply an implicit two-point backwards difference about $t = t^{n+1}$, which, after a rearrangement of terms, leads to
\begin{equation}
    \label{eq:BDF-1 semi-discrete diffusion}
    \left(\mathcal{I} - \frac{1}{\alpha^{2}} \Delta \right)\psi^{n+1} =  \psi^{n} + \Delta t S^{n+1}, 
\end{equation}
where we use $\alpha = 1/\sqrt{D \Delta t}$ for parabolic equations. Compare this with the definition of $\alpha$ in the semi-discrete wave equation immediately following \eqref{eq:modified helmholtz eqn}. Both cases involve a modified Helmholtz equation, but with different definitions of the scalar $\alpha$ and different ``right-hand sides." In places where it is not obvious, we shall distinguish the $\alpha$ associated with the wave equation from the diffusion equation through a subscript, with $\alpha_{W} = 1/(c\Delta t)$ being used for the wave equation and $\alpha_{D} = 1/\sqrt{D \Delta t}$ being used for the diffusion equation. The significance of the structural similarities between \eqref{eq:BDF-1 semi-discrete diffusion} the semi-discrete system \eqref{eq:BDF-1 semi-discrete phi}-\eqref{eq:BDF-1 semi-discrete A} ultimately permits the use of the same algorithms to invert the modified Helmholtz operator. Such similarities imply that the analytical differentiation formulas used in \cite{christlieb2024pic}, which were based on the integral solution to equation \eqref{eq:modified helmholtz eqn} are also valid.





==> 2-Formulation/Mapping-History.tex <==
\subsection{Charge and Current Mappings}
Above we considered the charge and current densities as moments of the distribution function $f_x$. With particle methods we view them as linear combinations of Dirac delta functions:

\begin{align} 
    \rho(\mathbf{x},t) &= \sum_{p=1}^{N_{p}} q_{p} \delta (\mathbf{x}-\mathbf{x}_{p}(t)), \label{eq:charge density}\\
    \mathbf{J}(\mathbf{x},t) & = \sum_{p=1}^{N_{p}} q_{p} \mathbf{v}_{p}(t) \delta (\mathbf{x}-\mathbf{x}_{p}(t)) \label{eq:current density}.
\end{align}

Here we have dropped the species subscript $s$ as each particle $p$ is individually considered. In a PIC framework we group sets of individual particles into ``clouds" of particles, or macroparticles, each with a macroparticle weight $w_{p}$. As such, we regularize the delta function into a shape function
\begin{align}
    \rho \left( \mathbf{x}, t \right) &= \sum_{p=1}^{N_{p}} q_{p} S \left(\mathbf{x} - \mathbf{x}_{p}(t) \right), \label{eq:PIC charge density} \\
    \mathbf{J} \left( \mathbf{x}, t \right) &= \sum_{p=1}^{N_{p}} q_{p} \mathbf{v}_{p}(t) S \left(\mathbf{x} - \mathbf{x}_{p}(t) \right), \label{eq:PIC current density}
\end{align}
where $q_{p} = w_{p} q_{p}$ is now defined to be the charge associated with a macroparticle. The shape functions $S$ dictate how we bring the charge and current of each macroparticle to the mesh. This mapping may be arbitrarily accurate, from nearest node to an order $N$ splines (see Figure \ref{fig:splines}).

The bilinear shape function (see Figure \ref{fig:Linear_Rho_Map}) is a common spline used to interpolate the charge. As an example, consider the two-dimensional case in which a particle is located at $(x_{p},y_{p})$, inside a cell with logical coordinates $$\left\{(x_{\ell}, y_{m})\right\}, \quad \ell = i,i+1, \quad m = j,j+1.$$ Let $f_{x} = \left(x_{p} - x_{i}\right)/(x_{i+1} - x_{i}))$ and $f_{y} = \left(x_{p} - y_{j}\right)/(y_{j+1} - y_{j}))$ denote the normalized distance of the particle from the left-most grid point in each direction. The charge that is assigned to each of the four grid vertices is given by
\begin{align}
    &Q_{i,j} = q_{p}(1-f_{x})(1-f_{y}), \\
    &Q_{i+1,j} = q_{p} f_{x}(1-f_{y}), \\
    &Q_{i,j+1} = q_{p}(1-f_{x})f_{y}, \\
    &Q_{i+1,j+1} = q_{p} f_{x} f_{y},
\end{align}
This is repeated for each particle $p$, with the charge at each cell being normalized by the corresponding cell volume $V_{i,j}$ in order to define the density $\rho_{i,j}$.

% The bilinear shape function (see Figure \ref{fig:Linear_Rho_Map}) is a common spline used to interpolate the charge. As an example, consider the two-dimensional case in which a particle is located at $(x_{p},y_{p})$, inside a cell having dimensions $(d_{x}, d_{y})$, with the bottom left node at location $(x,y)$. Let $w_{x} = \left(x_{p} - x\right)/d_{x}$ and $w_{y} = \left(y_{p} - y\right)/d_{y}$. The charge that is assigned to each of the four grid vertices, ordered counter-clockwise, is given by
% \begin{align}
%     &Q_1 = q_i(1-w_1)(1-w_2), \\
%     &Q_2 = q_i(w_1)(1-w_2), \\
%     &Q_3 = q_i(1-w_1)(w_2), \\
%     &Q_4 = q_i(w_1)(w_2),
% \end{align}
% We then compute $\rho = \frac{Q}{V}$, where $V$ is the volume of the cell.


In the following discussion we will briefly consider a few example charge and current mappings against which we may compare our map. 

\begin{figure}[h]
   \centering
    \includegraphics[clip, scale=0.75]{2-Formulation/figs/splines.png}
    \caption{Splines of zeroth (NGP), first (LS), second (QS), and third order (CS) \cite{JPVerboncoeur2005review}.}
    \label{fig:splines}
\end{figure}

\begin{figure}[h]
   \centering
    \includegraphics[clip, scale=0.75]{2-Formulation/figs/rho_scatter.jpg}
    \caption{A Linear Mapping \cite{JPVerboncoeur2005review}.}
    \label{fig:Linear_Rho_Map}
\end{figure}

\subsubsection{Electrostatics}
In modelling a plasma, we have $N_{p}$ (macro-)particles whose motion we wish to simulate. In the case of electrostatics, we are only interested in the electric field $\textbf{E}$, which we can compute from the potential $\textbf{E} = -\nabla\phi$. Computing the Coloumb potential for a particle requires us to examine the distance between that particle and every other particle in the system, and we need to do this for every particle, resulting in a $\mathcal{O}(N_{p}^{2})$ operation every timestep, which is simply not computationally tractable for even a modest count of particles. The alternative is to first map the charge of each particle to a $N^{d}$ mesh, where $d$ is the number of spatial dimensions and $N$ the number of points per dimension with $N \ll N_{p}$. The cost of this operation is $\mathcal{O}(N_{p})$. Then, the potential can be computed using a grid solver for Poisson's equation
$$
    -\Delta\phi = \frac{\rho}{\varepsilon_0}
$$
at a cost of $\mathcal{O}(N^{d})$ or even $\mathcal{O}(N^{d}\log{(N)})$ operations at each timestep. The combined approach scales as $\mathcal{O}((N_{p})$ since $N \ll N_{p}$. Once we acquire the potential, we acquire the electric field and interpolate it back to the particles, using it to compute their velocity. This procedure repeated with each iteration, so there is no need for divergence cleaning, as there is no way for leftover charge to remain on the mesh.


\subsubsection{Electromagnetics}

In the case of electromagnetic problems, things become more complicated. The use of a staggered Yee grid \cite{Yee1966}, allows one to automatically satisfy Gauss' law for the electric and magnetic fields when there are no free-charges. However, this choice introduces several complications. First, the adoption of a staggered mesh introduces complications for problems defined in non-trivial geometries. This is typically addressed by using a highly resolved uniform mesh to compensate for the ``staircase" that results along the boundaries \cite{JPVerboncoeur2004stairstep}. Conformal methods, which use curvilinear coordinate transformations to map the grid to one that is uniform \cite{reviewConformalPIC2015,WangConformalPIC2016}, have also been considered. Both approaches generally lead to a small time step due to the combination of small mesh cells and explicit timestepping. Second, the introduction of free-charges means that the usual guarantees for the Yee method no longer hold, so care must be taken when interpolating particle data to the grid to prevent the build-up of charge.

\begin{figure}[h]
   \centering
    \includegraphics[clip, scale=0.5]{2-Formulation/figs/Moving_Charge.jpg}
    \caption{A charge conserving map using a combination of zeroth and first order weighting.}
    \label{fig:charge-conserving-map}
\end{figure}

The Yee grid utilizes Maxwell's curl equations, so that only the current needs to be mapped to the grid. However, a naive bilinear interpolation of $\mathbf{J}$ does not preserve the continuity equation, which can lead to catastrophic errors in simulations of particle beams and pulsed power systems. This may be remedied with divergence cleaning \cite{Mardahl97conservation} or, alternatively, a more clever mapping scheme that combines piece-wise constant and linear spline interpolation that preserves these involutions \cite{VillasenorChargeConservation92}. Following the notation in \cite{JPVerboncoeur2005review}, if we take the weights $w_i$ defined above and define $\Delta \textbf{w} = \textbf{w}^{n+1} - \textbf{w}^{n}$ and $\bar{\textbf{w}} = \frac{\textbf{w}^n + \textbf{w}^{n+1}}{2}$, we acquire the following charge conserving map (in 2D):
\begin{align*}
    \begin{split}
        &I_{1,j+\frac{1}{2},k} = \frac{q_i}{\Delta t}\Delta w_1(1-\bar{w}_2), \\
        &I_{1,j+\frac{1}{2},k+1} = \frac{q_i}{\Delta t}\Delta w_1\bar{w}_2, \\
        &I_{2,j,k+\frac{1}{2}} = \frac{q_i}{\Delta t}(1-\bar{w}_1)\Delta w_2, \\
        &I_{2,j,k+\frac{1}{2}} = \frac{q_i}{\Delta t}\bar{w}_1\Delta w_2.
    \end{split}
\end{align*}
See figure \ref{fig:charge-conserving-map} for more details. Note if the particle crosses a cell border the path may be broken up and the process repeated for the constituent subpaths. In our case, we are considering a collocated mesh of vector and scalar potentials, as such we will need to consider an analogous way to preserve the continuity equation and thus the Lorenz gauge.

==> 2-Formulation/algorithm.tex <==
%
% Overview of the abstract algorithm we use
%
\subsection{The Algorithm}

We have described in the above sections the individual components of our algorithm. Stitching these components together is a relatively straightforward task, but one worth briefly discussing before providing the particular details of each method. If we consider Algorithm \ref{alg:IAEM-skeleton}, we see that we require two main components as with any PIC method: a solver for the fields and an advance for the particles. Additionally, we need a method of interpolating the fields to the particles and vice versa; these will be used by the particle pusher and the field solver, respectively. We already have our particle pusher in the form of the IAEM, and the way in which we interpolate the fields to the particles is the same throughout the proceeding discussion, namely a simple bilinear map. We are primarily interested in the ways of acquiring $\rho$, as well as the ways we can obtain the potentials and their derivatives in the simulation (lines \ref{alg:step-charge-den-naive}, \ref{alg:step-potentials-naive}, \ref{alg:step-potential-derivatives-naive}). The specific details associated with these components is the subject of the sections \ref{sec:3 exact charge maps} and \ref{sec:4 gauge correcting}.

==> 3-Exact-Maps/gauss-law.tex <==
\subsection{Satisfying Gauss' Law}

A benefit that comes with satisfying the semi-discrete Lorenz gauge \eqref{eq:semi-discrete Lorenz} is the corresponding satisfaction of Gauss' law \eqref{eq:Gauss-E}. We show this as follows:

\begin{theorem}
    If \eqref{eq:semi-discrete Lorenz} is satisfied, then \eqref{eq:Gauss-E} is satisfied.
\end{theorem}

\begin{proof}
    Consider a backward Euler discretization of the Lorenz gauge condition in time:
    \begin{equation}
        \frac{1}{c^2}\frac{\phi^{n+1} - \phi^{n}}{\Delta t} + \nabla \cdot \textbf{A}^{n+1} = 0.
    \end{equation}
    We know from \eqref{eq:Convert potentials to EB} that
    \begin{equation}
        \textbf{E}^{n} = -\nabla\phi^{n} - \frac{\textbf{A}^{n+1} - \textbf{A}^n}{\Delta t}.
    \end{equation}
    Applying the divergence to both sides of this definition yields
    \begin{align}
        \begin{split}
            \nabla \cdot \textbf{E}^{n} &= -\Delta \phi^{n} - \frac{\nabla\cdot\textbf{A}^{n+1} - \nabla\cdot\textbf{A}^{n}}{\Delta t} \\
            &= -\Delta\phi^{n} - \frac{\left(-\frac{1}{c^2}\frac{\phi^{n+1} - \phi^{n}}{\Delta t}\right) - \left(-\frac{1}{c^2}\frac{\phi^{n} - \phi^{n-1}}{\Delta t}\right)}{\Delta t}\\
            &= -\Delta \phi^{n} + \frac{1}{c^2}\frac{\phi^{n+1} - 2\phi^{n} + \phi^{n-1}}{\Delta t^2}.
        \end{split}
    \end{align}
    This is the backward Euler discretization of \eqref{eq:scalar potential eqn lorenz}, ie \eqref{eq:BDF-1 semi-discrete phi}, and is therefore equal to $\frac{\rho^{n+1}}{\epsilon_0}$.
\end{proof}

It is worth noting that the discrete time derivative operator applied to the Lorenz gauge must be the same as that applied to the scalar potential wave equation.

==> 4-Approximate-Maps/algorithm.tex <==
%
% Section that describes the algorithm
%
\subsection{Remarks on the Algorithm}
\label{subsec:4 parabolic cleaning alg}

In the formulation used in the parabolic cleaning method, the wave equations for the potentials $\phi$ and $\mathbf{A}$ (respectively equations \eqref{eq: modified scalar potential eqn lorenz parabolic system} and \eqref{eq:vector potential eqn lorenz parabolic system}) are coupled to the parabolic equation for the Lagrange multiplier $\psi$. The solution to the wave equation for the scalar potential $\phi$ depends on the Laplacian of the Lagrange multiplier $\psi$, and the function $\psi$ is obtained from the solution of a parabolic equation, which itself, requires knowledge of the potentials. We propose to deal with this coupling in the following way. Suppose we are given the particle data $\rho^{n+1}$ and $\mathbf{J}^{n+1}$. Then we perform the following steps:
\begin{enumerate}
    \item Perform the BDF advance for $\mathbf{A}^{n+1}$ and $\nabla \mathbf{A}^{n+1}$ using the current density $\mathbf{J}^{n+1}$.
    \item Approximate $\partial_{t} \left( \nabla \cdot \mathbf{A}^{n+1}\right)$ using backwards differences for the time derivative.
    \item Compute $\phi^{n+1}$ and its Laplacian $\Delta \phi^{n+1}$ from $\Delta \psi^{n}$ and the charge density $\rho^{n+1}$.
    \item Compute $\psi^{n+1}$ and its Laplacian $\Delta \psi^{n+1}$ using $\Delta \phi^{n+1}$ and the approximation for $\partial_{t} \left( \nabla \cdot \mathbf{A}^{n+1}\right)$.
    \item Recompute the scalar potential $\phi^{n+1}$ and its Laplacian $\Delta \phi^{n+1}$ from $\Delta \psi^{n+1}$ and the charge density $\rho^{n+1}$.
    \item Repeat steps 3 - 5 until converged.
\end{enumerate}


The BDF method for the scalar wave equation, discussed in our previous paper \cite{christlieb2024pic}, approximates the second-order time derivative using a total of three levels in time. This modification requires additional storage for $\Delta \phi^{n+1}$, $\Delta \psi^{n+1}$, as well as the time derivative $\partial_{t} \left( \nabla \cdot \mathbf{A}^{n+1}\right)$. We only need to store the Laplacian terms at a single time level, since these terms can be updated in-place. The number of time levels needed to approximate $\partial_{t} \left( \nabla \cdot \mathbf{A}^{n+1}\right)$ depends on accuracy requirements. For first-order time accuracy, which is consistent with the BDF scheme used to evolve the fields, it is enough to store two levels, namely $\nabla \cdot \mathbf{A}^{n}$ and $\nabla \cdot \mathbf{A}^{n+1}$. Although we have written the method in the form of an iterative scheme, we choose to perform a single pass of steps 3-5, since this is designed to be an approximate method. In general, however, these steps can be performed until some convergence criteria is met, e.g., the changes between iterates for $\phi^{n+1}$ become sufficiently small. Lastly, we have not yet described the way in which the Laplacian terms $\Delta \phi^{n+1}$ and $\Delta \psi^{n+1}$ are approximated. In our previous paper \cite{christlieb2024pic}, the spatial derivatives were calculated by taking analytical derivatives of the integral solution. These derivatives were shown to converge at the same rates as the fields, but with different error constants. 
% We discuss two approaches to approximate second-order spatial derivatives in Appendix \ref{app:Laplacian}. 
While we have investigated extensions of these methods to the case of second derivatives, the overall size of the error is not reasonable for the first-order BDF method and the range of time step sizes considered in this paper. We do not expect this to be an issue for higher-order time accurate BDF field solvers (e.g., the second-order BDF method in \cite{causley2017wave-propagation}) as the error constant for these methods is much smaller. Since we are focused on the formulation and not considering geometry in this work, it is sufficient to approximate the Laplacians using second-order accurate finite-differences.

In this section we introduced a more involved method of cleaning $\phi$ by adding a diffusivity coefficient, $\psi$. This method is designed to leave lines \ref{alg:step-charge-den-naive} and \ref{alg:step-current-den-naive} alone and modify the BDF method found in lines \ref{alg:step-potentials-naive} and \ref{alg:step-potential-derivatives-naive}. The modified BDF method will also be applied to $\psi$, in addition to computing its Laplacian and that of $\phi$. The sequencing of this is more involved than the methods previously described, and the details of this subroutine are described in Algorithm \ref{alg:parabolic-subroutine}.

% \begin{enumerate}
%     \item Compute $S_{\textbf{A}^{(1)}} \coloneqq \mu_0\textbf{J}^{(1)}$ and $S_{\textbf{A}^{(2)}} \coloneqq \mu_0\textbf{J}^{(2)}$.
%     \item Apply BDF to $\textbf{A}^{(1)}$ and $\textbf{A}^{(2)}$ using $S_{\textbf{A}^{(1)}}$ and $S_{\textbf{A}^{(2)}}$ as their sources, respectively.
%     \item Compute $S_{\phi,1} \coloneqq \frac{\rho}{\epsilon_0} + D\Delta\psi$.
%     \item Apply BDF to $\phi$ using $S_{\phi,1}$ as its source.
%     \item Numerically compute $\Delta \phi$ using a basic finite difference scheme.
%     \item Numerically compute the time derivative of $\nabla \cdot \textbf{A}$ using a basic finite difference scheme.
%     \item Compute $S_\psi \coloneqq \Delta\phi + \frac{\rho}{\epsilon_0} + \frac{1}{D}\frac{\partial}{\partial t}\left(\nabla \cdot \textbf{A}\right)$.
%     \item Apply BDF to $\psi$ using $S_\psi$ as its source.
%     \item Compute $S_{\phi,2} \coloneqq \frac{\rho}{\epsilon_0} + D\Delta\psi$.
%     \item Apply BDF again to $\phi$ using $S_{\phi,2}$ as the source function.
% \end{enumerate}

\begin{algorithm}[t]
    \caption{Subroutine replacing lines \ref{alg:step-potentials-naive} and \ref{alg:step-potential-derivatives-naive} of Algorithm \ref{alg:IAEM-skeleton}.}
    \label{alg:parabolic-subroutine}
    \begin{algorithmic}[1]
        \State \textbf{Given}: $\textbf{J}^{n+1}$, $\rho^{n+1}$, $\textbf{A}^{n}$, $\phi^{n}$, and $\psi^{n}$.
        
        \vspace{10pt}
        
        \State $S_{A^{(1)}}^{n+1} \gets \mu_0 J^{(1),n+1}$, $S_{A^{(2)}}^{n+1} \gets \mu_0 J^{(2),n+1}$.
    
        \State Using BDF compute $A^{(1),n+1}$ and $A^{(1),n+1}$ from $A^{(1),n}$ and $A^{(2),n}$ using $S_{A^{(1)}}^{n+1}$ and $S_{A^{(2)}}^{n+1}$ as their sources, respectively.
        
        \State $S_{\phi,1}^{n+1} \gets \frac{\rho^{n+1}}{\epsilon_0} + D\Delta \psi^{n}$.
        
        \State Using BDF compute $\Tilde{\phi}^{n+1}$ from $\phi^{n}$ using $S_{\phi,1}^{n+1}$ as its source.
        
        \State Numerically compute $\Delta \Tilde{\phi}^{n+1}$ using a basic finite difference scheme.

        \State Numerically compute $\frac{\partial}{\partial t}\nabla \cdot \textbf{A}^{n+1}$ using a basic finite difference scheme.
    
        \State $S_{\psi}^{n+1} \gets \Delta \Tilde{\phi}^{n+1} + \frac{\rho^{n+1}}{\epsilon_0} + \frac{1}{D}\frac{\partial}{\partial t}\left(\nabla \cdot \textbf{A}^{n+1}\right)$.
        
        \State Using BDF compute $\psi^{n+1}$ from $\psi^{n}$ using $S_{\psi}^{n+1}$ as its source.
        
        \State $S_{\phi,2} \gets \frac{\rho^{n+1}}{\epsilon_0} + D\Delta \psi^{n+1}$.
        
        \State Using BDF compute $\phi^{n+1}$ from $\Tilde{\phi}^{n+1}$ using $S^{n+1}_{\phi,2}$ as the source function.
    
    \end{algorithmic}
\end{algorithm}

==> 4-Approximate-Maps/cleaning.tex <==
\subsection{A Modified Lorenz Gauge Formulation with Parabolic Gauge Cleaning}
\label{subsec:Maxwell Lorenz with parabolic cleaning}


To develop the auxiliary equation, we first modify the Lorenz gauge condition by introducing a function $\psi$ according to
\begin{equation}
    \frac{1}{c^2} \partial_{t} \phi + \nabla \cdot \mathbf{A} = \psi.
    \label{eq:modified Lorenz gauge}
\end{equation}
The function $\psi$ represents a Lagrange multiplier for the Lorenz gauge condition \eqref{eq:Lorenz gauge condition}, which is a constraint to be satisfied. This function should not be thought of as a generalized gauge condition. We connect this auxiliary function to the Lorenz gauge formulation by modifying the equation for the scalar potential \eqref{eq:scalar potential eqn lorenz} as follows:
\begin{equation} 
\frac{1}{c^2} \partial_{tt} \phi -\Delta \phi= D \Delta \psi + \frac{1}{\epsilon_{0}} \rho, \label{eq:scalar potential eqn lorenz modified}
\end{equation}
Here $D > 0$ is a diffusivity parameter whose value will be specified at a later time. Note that when the residual satisfies $\psi \equiv 0$, we recover the original equation \eqref{eq:scalar potential eqn lorenz}.

Next, we derive a parabolic equation for the Lagrange multiplier $\psi$. Taking the time derivative of equation \eqref{eq:modified Lorenz gauge}, we obtain
\begin{equation*}
    \partial_{t} \psi = \frac{1}{c^2} \partial_{tt} \phi + \partial_{t} \left(\nabla \cdot \mathbf{A} \right).
\end{equation*}
Combining this result with the modified equation \eqref{eq:scalar potential eqn lorenz modified} for the scalar potential results in a parabolic equation of the form
\begin{equation*}
    \partial_{t} \psi -  D \Delta \psi = \Delta \phi + \frac{1}{\epsilon_{0}} \rho + \partial_{t} \left(\nabla \cdot \mathbf{A} \right).
\end{equation*}
In the limiting case where $D \rightarrow 0^{+}$, the steady-state for the above parabolic equation is the elliptic equation
\begin{equation*}
    - \Delta \phi = \frac{1}{\epsilon_{0}} \rho + \partial_{t} \left(\nabla \cdot \mathbf{A} \right).
\end{equation*}
This equation for $\phi$ was used in \cite{wolf2016particle} to ensure the satisfaction of Gauss' law $\nabla \cdot \mathbf{E} = \rho/\epsilon_{0}$, and can be derived directly from the definitions presented in equation \eqref{eq:Convert potentials to EB}. The terms on the right-hand side represent the residual for Gauss' law and act as a source in the parabolic (or elliptic) equation for $\psi$. Consequently, if the potentials $\phi$ and $\mathbf{A}$ satisfy Gauss' law, so that charge is conserved, then the function $\psi$ vanishes, and the Lorenz gauge condition \eqref{eq:Lorenz gauge condition} is satisfied. The modified system that needs to be solved is 
\begin{empheq}[left=\empheqlbrace]{align}
    &\frac{d\mathbf{x}_{i}}{dt} = \frac{c^2 \left(\mathbf{P}_{i} - q_{i}\mathbf{A}\right)}{\sqrt{c^2\left(\mathbf{P}_{i} - q_{i} \mathbf{A}\right)^2 + \left(m_{i} c^2\right)^2}}, \label{eq:Position equation relativistic form parabolic system} \\
    &\frac{d\mathbf{P}_{i}}{dt} = -q_{i} \nabla \phi + \frac{q_{i} c^2 \left( \nabla\mathbf{A}\right) \cdot \left(\mathbf{P}_{i} - q_{i}\mathbf{A}\right)}{\sqrt{c^2\left(\mathbf{P}_{i} - q_{i} \mathbf{A}\right)^2 + \left(m_{i} c^2\right)^2}}, \label{eq:Generalized momentum equation relativistic form parabolic system} \\
    &\frac{1}{c^2} \partial_{tt} \phi -\Delta \phi = D \Delta \psi + \frac{1}{\epsilon_{0}} \rho, \label{eq: modified scalar potential eqn lorenz parabolic system} \\ 
    &\frac{1}{c^2} \partial_{tt} \mathbf{A} -\Delta \mathbf{A}= \mu_{0} \mathbf{J}, \label{eq:vector potential eqn lorenz parabolic system} \\ 
    &\partial_{t} \psi -  D \Delta \psi = \Delta \phi + \frac{1}{\epsilon_{0}} \rho + \partial_{t} \left(\nabla \cdot \mathbf{A} \right) \label{eq:parabolic equation psi parabolic system},
\end{empheq}
where $D > 0$ and $i = 1, 2, \cdots, N_{p}$ is the particle index. As before, the potentials in the particle equations are evaluated at the position of the corresponding particle.



==> 4-Approximate-Maps/introduction.tex <==
%
% Section that holds the details of the approximate map
%
\section{Correcting the Potentials to Enforce the Lorenz Gauge}
\label{sec:4 gauge correcting}

In this section, we introduce a correction technique to enforce a semi-discrete Lorenz gauge condition.  This uses the semi-discrete gauge condition to correct the scalar potential in a direct manner, which results in a point-wise consistent set of field variables.  This method can be used to define a corrected charge density satisfying the continuity equation if one needs the exact charge density, $\rho$.  It should be noted that a potential drawback of the method presented in this section is its adaption to satisfy Gauss' law, which will require additional work beyond what is presented here.

==> 4-Approximate-Maps/main4.tex <==
%
% Section introduction
%
\input{4-Approximate-Maps/introduction}

%
% Section on the cleaning formulation
%
% \input{4-Approximate-Maps/cleaning}

% %
% % Section on the boundary conditions for psi
% %
% \input{4-Approximate-Maps/psi_boundary_conditions}

% %
% % Section on the cleaning algorithm
% %
% \input{4-Approximate-Maps/algorithm}

%
% Summary of section content
%
\input{4-Approximate-Maps/summary}

==> 4-Approximate-Maps/psi_boundary_conditions.tex <==
%
% Section that holds the details of the boundary conditions
%
\subsection{Boundary Conditions for the Parabolic Equation and Limiting Behavior}
\label{subsec:4 parabolic cleaning psi BCs}

To solve the parabolic equation \eqref{eq:parabolic equation psi parabolic system} on bounded domains, we prescribe the following initial and boundary data on the Lagrange multiplier $\psi$:
\begin{align*}
    \psi(\mathbf{x},0) &= 0, \quad \mathbf{x} \in \Omega, \\
    \psi(\mathbf{x},t) &= 0, \quad \left( \mathbf{x},t\right) \in \partial \Omega \times \mathbb{R}^{+}.
\end{align*}
At time $t = 0$, the initial data for the potentials $\phi$ and $\mathbf{A}$ is assumed to satisfy the Lorenz gauge condition \eqref{eq:Lorenz gauge condition}, so $\psi = 0$.

Since the parabolic equation for the Lagrange multiplier is linear, its behavior can be understood in the sense of separation of variables. First, let $\left\{\lambda_{n},\varphi_{n} \left( \mathbf{x}\right) \right\}_{n = 1}^{\infty}$ denote the set of (orthogonal) eigenvalues and eigenfunctions for the eigenvalue problem
\begin{equation}
    \label{eq:Eigenvalue problem Laplacian}
    -\Delta \varphi_{n} = \lambda_{n} \varphi_{n}.
\end{equation}
It is essential to note that the eigenvalues $\lambda_{n}$ are, in general, non-negative. To simplify the notation we introduce the function
\begin{equation*}
    Q\left( \mathbf{x},t\right) = \Delta \phi + \frac{1}{\epsilon_{0}} \rho + \partial_{t} \left(\nabla \cdot \mathbf{A} \right).
\end{equation*}
Each of these functions can be expanded in terms of the eigenbasis $\varphi$, so that
\begin{equation*}
    \psi \left( \mathbf{x},t\right) = \sum_{n = 0}^{\infty} \psi_{n} (t) \varphi_{n} \left( \mathbf{x} \right), \quad Q\left( \mathbf{x},t\right) = \sum_{n = 0}^{\infty} Q_{n} (t) \varphi_{n} \left( \mathbf{x} \right).
\end{equation*}
Substituting these expansions into the parabolic equation \eqref{eq:parabolic equation psi parabolic system} and using the property \eqref{eq:Eigenvalue problem Laplacian}, in addition to orthogonality, we can obtain the system of ODEs
\begin{empheq}[left=\empheqlbrace]{align*}
    &\frac{d\psi_{n}}{dt} + D \lambda_{n} \psi_{n} = Q_{n}, \quad n = 0, 1, \cdots \\
    &\psi_{n}(0) = 0.
\end{empheq}
An application of the integrating factor method yields the solution
\begin{equation*}
    \psi_{n}(t) = \int_{0}^{t} e^{D\lambda_{n}(\tau - t)} Q_{n}(\tau) \,d\tau, \quad n = 0, 1, \cdots.
\end{equation*}
If the coefficients of the source $Q_{n}$ are compactly supported in time, then for any $D > 0$, the coefficients satisfy
\begin{equation*}
    \lim_{t \to \infty} \psi_{n}(t) = 0, \quad n = 0, 1, \cdots.
\end{equation*}
In the problems that we consider, the source function $Q$ does not have this property. However, for a sufficiently large $D > 0$, these coefficients remain bounded, which provides the mechanism to control the errors in the Lorenz gauge condition.





==> 4-Approximate-Maps/summary.tex <==
%
% Summary of the section contents
%
\subsection{Summary}
\label{subsec:4 Summary}

\begin{table}[!htb]
    \centering
    \def\arraystretch{1.2}
    \begin{tabular}{ | c || c | }
        \hline
        \textbf{Method}  & \textbf{Changes} \\
        \hline
        Numerical Derivatives & Lines \ref{alg:step-current-den-naive} and \ref{alg:step-potential-derivatives-naive} \\
        %\hline
        Multi-dimensional Boundary Integral & Lines \cancel{\ref{alg:step-charge-den-naive}},  \ref{alg:step-potentials-naive}, and \ref{alg:step-potential-derivatives-naive} \\
        %\hline
        Correcting $\phi$ & Add line to correct $\phi$ after \ref{alg:step-potential-derivatives-naive}. \\
        \hline
    \end{tabular}
    \caption{The three methods we introduce and how they change Algorithm \ref{alg:IAEM-skeleton}.}
    \label{tab:algorithm modifications}
\end{table}

In this section, we introduced a correction to $\phi$ based on the gauge condition. This is the least intrusive of all our methods, being accomplished by simply adding a line after \ref{alg:step-potential-derivatives-naive} in which we compute the correction to $\phi$ and its numerical derivatives.  The changes made to Algorithm \ref{alg:IAEM-skeleton} for all three methods are summarized in Table \ref{tab:algorithm modifications}.  In the next section, we investigate the capabilities of the exact and approximate methods in problems defined on periodic domains.

==> 5-Algorithm-Overview/algorithms.tex <==
\subsection{Charge Conserving Modifications}

The modifications we make to Algorithm \ref{alg:IAEM} are thankfully straightforward. First, the above relies on a naive bilinear interpolation of both $\textbf{J}^{n+1}$ and $\rho^{n+1}$. Alternatively, as we described in Section \ref{subsec:3-charge-conserving-numerical-derivatives} we can modify Line \ref{alg:step-charge-den} to use the semi-discrete continuity equation \eqref{eq:semi-discrete continuity equation} to acquire $\rho^{n+1}$ using the FFT, FD6, or any other standard numerical derivative operator. Doing so we must take care to acquire $\nabla \textbf{A}^{n+1}$ and $\nabla \phi^{n+1}$ in an identical manner on Line \ref{alg:step-potentials}, neglecting to do so resulting in an unsatisfied gauge condition.

If we are to use the multi-dimensional boundary integral solution described in \ref{subsec:3-charge-conserving-boundary-integral-solution}, then we forego modifying Line \ref{alg:step-charge-den} and instead change Line \ref{alg:step-potentials}, computing $\phi^{n+1}$ according to the boundary integral solution \eqref{eq:phi BIE with map} (note the computation of $\textbf{A}^{n+1}$ is not altered). This has yet to be implemented and will be the subject of future inquiry.

% \subsection{Gauge Enforcement}

% The other approach is to forego ensuring the satisfaction of the semi-discrete continuity equation and instead correct the gauge condition after the fact. For the first approach, we simply add a step immediately after Line \ref{alg:step-potentials}. We call the potential we acquire from Line \ref{alg:step-potentials} $\phi_A^{n+1}$ and proceed to compute $\phi_C^{n+1}$, adding this to $\phi_A^{n+1}$, resulting in $\phi_{C}^{n+1}$ as described in \ref{subsec:corrected_phi}.

% \begin{algorithm}[t]
%     \caption{Outline of the PIC algorithm with the improved asymmetric Euler method (IAEM)}
%     Perform one time step of the PIC cycle using the improved asymmetric Euler method. 
%     \label{alg:IAEM}
%     \begin{algorithmic}[1]
%     \State \textbf{Given}: $(\mathbf{x}_{i}^{0}, \mathbf{P}_{i}^{0}, \mathbf{v}_{i}^{0})$, as well as the fields $ \left( \phi^{0}, \nabla \phi^{0} \right)$ and $\mathbf{A}^{0}, \nabla \mathbf{A}^{0}$
%     \State Initialize $\mathbf{v}_{i}^{-1} = \mathbf{v}_{i}(-\Delta t)$ using a Taylor approximation.
%     \While{stepping}
    
%     \vspace{10pt}
    
%     \State \label{start time loop} Update the particle positions with $$\mathbf{x}_{i}^{n+1} = \mathbf{x}_{i}^{n} + \mathbf{v}_{i}^{n} \Delta t.$$
    
%     \State Using the position data $\mathbf{x}_{i}^{n+1}$ and velocity data $\mathbf{v}_{i}^{n}$, compute the current density $$\tilde{\mathbf{J}}^{n+1} = \mathbf{J}^{n+1} + \mathcal{O}(\Delta t).$$
    
%     \State Using the position data $\mathbf{x}_{i}^{n+1}$, compute the charge density $\rho^{n+1}$. \label{alg:step-charge-den}
    
%     \State Compute the potentials and their derivatives at time level $t^{n+1}$ using the BDF field solver. \label{alg:step-potentials}

%     \State Evaluate the Taylor corrected particle velocities $$\mathbf{v}_{i}^{*} = 2 \mathbf{v}_{i}^{n} - \mathbf{v}_{i}^{n-1}.$$
    
%     \State Calculate the new generalized momentum according to $$\mathbf{P}_{i}^{n+1} = \mathbf{P}_{i}^{n} + q_i \Big( - \nabla \phi^{n+1} + \nabla \mathbf{A}^{n+1} \cdot \mathbf{v}_{i}^{*} \Big)\Delta t.$$
    
%     \State Convert the new generalized momenta into new particle velocities with $$ \mathbf{v}_{i}^{n+1} =  \frac{c^2 \left( \mathbf{P}_{i}^{n+1} - q_{i} \mathbf{A}^{n+1}\right)}{\sqrt{ c^2\left( \mathbf{P}_{i}^{n+1} - q_{i} \mathbf{A}^{n+1}\right)^2 + \left(m_{i}c^2\right)^2}}. $$
    
%     \State Shift the time history data and return to step \ref{start time loop} to begin the next time step. 
    
%     \EndWhile
%     \end{algorithmic}
% \end{algorithm}

==> 5-Algorithm-Overview/introduction.tex <==
\section{Algorithm Overview}\label{sec:Algorithm}

In the preceding sections we sketched out a set of techniques to solve both the particle motion and the field updates. We will now take a brief moment to summarize this in terms of a more concrete algorithm in the spirit of what we previously laid out in \cite{christlieb2024pic}.

==> 5-Algorithm-Overview/main5.tex <==
%
% Section introduction
%
\input{5-Algorithm-Overview/introduction}

%
% Overview of the algorithm and how the various pieces fit in.
%
\input{5-Algorithm-Overview/algorithms}
